Dependence structure estimation using Copula Recursive Trees

We construct the COpula Recursive Tree (CORT) estimator: a flexible, consistent, piecewise linear estimator of a copula, leveraging the patchwork copula formalization and various piecewise constant density estimators. While the patchwork structure imposes a grid, the CORT estimator is data-driven and constructs the (possibly irregular) grid recursively from the data, minimizing a chosen distance on the copula space. The addition of the copula constraints makes usual density estimators unusable, whereas the CORT estimator is only concerned with dependence and guarantees the uniformity of margins. Refinements such as localized dimension reduction and bagging are developed, analyzed, and tested through simulated data.

==> clayton_table_bagging_result.tex <==
\begin{table}[H]

\caption{\label{tab:clayton_table_bagging_result}Results of the bagging of each model on Dataset \ref{data:clayton}}
\centering
\begin{tabu} to \linewidth {>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X}
\toprule
  & Empirical & Cb(m=10) & Cb(m=5) & Beta & Cort\\
\midrule
$\hat{J}(\hat{c}_{\Gras{\omega}})$ & 0.00501 & -9.27 & -7.69 & 120 & \textbf{-54.6}\\
$\hat{K}(\hat{c}_{\Gras{\omega}})$ & Inf & Inf & Inf & -0.582 & \textbf{-1.97}\\
$\hat{M}(\hat{c}_{\Gras{\omega}})$ & 2.84e-05 & \textbf{2.51e-05} & 5.25e-05 & 3.38e-05 & 9.41e-05\\
$\hat{N}(\hat{c}_{\Gras{\omega}})$ & -0.000666 & \textbf{-0.000669} & -0.000641 & -0.000657 & -0.000639\\
\bottomrule
\end{tabu}
\end{table}


==> clayton_table_cramer.tex <==
\begin{table}[H]

\caption{\label{tab:clayton_table_cramer}$\hat{P}$ error statistics for Dataset \ref{data:clayton}}
\centering
\begin{tabu} to \linewidth {>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X}
\toprule
  & Empirical & Cb(m=10) & Cb(m=5) & Beta & Cort & Cort Forest\\
\midrule
Mean & 7.42e-05 & \textbf{5.16e-05} & 7.54e-05 & 5.32e-05 & 2.46e-04 & 6.96e-05\\
Sd & 2.01e-05 & \textbf{1.12e-05} & 1.80e-05 & 1.76e-05 & 3.64e-04 & 2.92e-05\\
\bottomrule
\end{tabu}
\end{table}


==> clayton_table_dep_mes.tex <==
\begin{table}[H]

\caption{\label{tab:clayton_table_dep_mes}Obtained dependence measures of several models on Dataset \ref{data:clayton}}
\centering
\begin{tabu} to \linewidth {>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X}
\toprule
  & Empirical & Cb(m=10) & Cb(m=5) & Beta & Cort & Bagged Cort\\
\midrule
\addlinespace[0.3em]
\multicolumn{7}{l}{\textbf{Kendall Taus}}\\
\hspace{1em}$\tau_{1,2}$ & -0.003 & 0.010 & 0.006 & -0.014 & 0.000 & -0.020\\
\hspace{1em}$\tau_{1,3}$ & -0.796 & -0.750 & -0.673 & -0.799 & -0.780 & -0.493\\
\hspace{1em}$\tau_{1,4}$ & 0.779 & 0.732 & 0.659 & 0.779 & 0.707 & 0.474\\
\hspace{1em}$\tau_{2,3}$ & 0.015 & 0.010 & 0.011 & 0.029 & 0.000 & 0.031\\
\hspace{1em}$\tau_{2,4}$ & -0.024 & -0.009 & -0.010 & -0.038 & 0.000 & -0.045\\
\hspace{1em}$\tau_{3,4}$ & -0.775 & -0.728 & -0.654 & -0.773 & -0.695 & -0.566\\
\addlinespace[0.3em]
\multicolumn{7}{l}{\textbf{Spearman Rhos}}\\
\hspace{1em}$\rho_{1,2}$ & -0.005 & 0.013 & 0.010 & -0.023 & 0.000 & -0.029\\
\hspace{1em}$\rho_{1,3}$ & -0.934 & -0.915 & -0.868 & -0.936 & -0.926 & -0.648\\
\hspace{1em}$\rho_{1,4}$ & 0.924 & 0.903 & 0.857 & 0.925 & 0.872 & 0.626\\
\hspace{1em}$\rho_{2,3}$ & 0.023 & 0.014 & 0.016 & 0.045 & 0.000 & 0.047\\
\hspace{1em}$\rho_{2,4}$ & -0.035 & -0.016 & -0.016 & -0.057 & 0.000 & -0.068\\
\hspace{1em}$\rho_{3,4}$ & -0.922 & -0.901 & -0.853 & -0.922 & -0.862 & -0.735\\
\bottomrule
\end{tabu}
\end{table}


==> funcdep_table_bagging_result.tex <==
\begin{table}[H]

\caption{\label{tab:funcdep_table_bagging_result}Results of the bagging of each model on Dataset \ref{data:funcdep}}
\centering
\begin{tabu} to \linewidth {>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X}
\toprule
  & Empirical & Cb(m=10) & Cb(m=5) & Beta & Cort\\
\midrule
$\hat{J}(\hat{c}_{\Gras{\omega}})$ & 0.002 & -15.7 & -7.22 & -23 & \textbf{-23.3}\\
$\hat{K}(\hat{c}_{\Gras{\omega}})$ & Inf & -2.52 & -1.79 & \textbf{-3.12} & -1.72\\
$\hat{M}(\hat{c}_{\Gras{\omega}})$ & \textbf{1.69e-05} & 0.000172 & 0.000736 & 4.76e-05 & 0.00233\\
$\hat{N}(\hat{c}_{\Gras{\omega}})$ & \textbf{-0.0201} & -0.0199 & -0.0194 & -0.0201 & -0.0177\\
\bottomrule
\end{tabu}
\end{table}


==> funcdep_table_cramer.tex <==
\begin{table}[H]

\caption{\label{tab:funcdep_table_cramer}$\hat{P}$ error statistics for Dataset \ref{data:funcdep}}
\centering
\begin{tabu} to \linewidth {>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X}
\toprule
  & Empirical & Cb(m=10) & Cb(m=5) & Beta & Cort & Cort Forest\\
\midrule
Mean & \textbf{8.34e-05} & 2.06e-04 & 7.39e-04 & 9.44e-05 & 2.77e-03 & 2.79e-03\\
Sd & \textbf{5.88e-05} & 1.42e-04 & 2.40e-04 & 8.84e-05 & 2.12e-03 & 8.94e-04\\
\bottomrule
\end{tabu}
\end{table}


==> funcdep_table_dep_mes.tex <==
\begin{table}[H]

\caption{\label{tab:funcdep_table_dep_mes}Obtained dependence measures of several models on Dataset \ref{data:funcdep}}
\centering
\begin{tabu} to \linewidth {>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X}
\toprule
  & Empirical & Cb(m=10) & Cb(m=5) & Beta & Cort & Bagged Cort\\
\midrule
\addlinespace[0.3em]
\multicolumn{7}{l}{\textbf{Kendall Taus}}\\
\hspace{1em}$\tau_{1,2}$ & -0.495 & -0.491 & -0.471 & -0.500 & -0.458 & -0.451\\
\hspace{1em}$\tau_{1,3}$ & 0.089 & 0.042 & -0.002 & 0.084 & 0.171 & 0.048\\
\hspace{1em}$\tau_{2,3}$ & 0.005 & 0.015 & 0.004 & 0.007 & -0.109 & 0.013\\
\addlinespace[0.3em]
\multicolumn{7}{l}{\textbf{Spearman Rhos}}\\
\hspace{1em}$\rho_{1,2}$ & -0.743 & -0.737 & -0.715 & -0.747 & -0.713 & -0.674\\
\hspace{1em}$\rho_{1,3}$ & -0.156 & -0.154 & -0.146 & -0.159 & 0.246 & 0.060\\
\hspace{1em}$\rho_{2,3}$ & -0.019 & 0.012 & -0.001 & -0.010 & -0.177 & 0.020\\
\bottomrule
\end{tabu}
\end{table}


==> impossible_table_bagging_result.tex <==
\begin{table}[H]

\caption{\label{tab:impossible_table_bagging_result}Results of the bagging of each model on Dataset \ref{data:impossible}}
\centering
\begin{tabu} to \linewidth {>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X}
\toprule
  & Empirical & Cb(m=10) & Cb(m=5) & Beta & Cort\\
\midrule
$\hat{J}(\hat{c}_{\Gras{\omega}})$ & 0.00501 & -1.48 & -1.39 & -1.21 & \textbf{-2.55}\\
$\hat{K}(\hat{c}_{\Gras{\omega}})$ & Inf & -0.346 & -0.271 & \textbf{-0.426} & -0.311\\
$\hat{M}(\hat{c}_{\Gras{\omega}})$ & \textbf{3.03e-05} & 5.16e-05 & 0.00016 & 7.38e-05 & 0.000907\\
$\hat{N}(\hat{c}_{\Gras{\omega}})$ & \textbf{-0.134} & -0.134 & -0.134 & -0.134 & -0.134\\
\bottomrule
\end{tabu}
\end{table}


==> impossible_table_cramer.tex <==
\begin{table}[H]

\caption{\label{tab:impossible_table_cramer}$\hat{P}$ error statistics for Dataset \ref{data:impossible}}
\centering
\begin{tabu} to \linewidth {>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X}
\toprule
  & Empirical & Cb(m=10) & Cb(m=5) & Beta & Cort & Cort Forest\\
\midrule
Mean & 0.000239 & \textbf{0.000198} & 0.000284 & 0.000213 & 0.001430 & 0.000567\\
Sd & 0.000127 & 0.000113 & \textbf{0.000111} & 0.000121 & 0.000786 & 0.000185\\
\bottomrule
\end{tabu}
\end{table}


==> impossible_table_dep_mes.tex <==
\begin{table}[H]

\caption{\label{tab:impossible_table_dep_mes}Obtained dependence measures of several models on Dataset \ref{data:impossible}}
\centering
\begin{tabu} to \linewidth {>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X}
\toprule
  & Empirical & Cb(m=10) & Cb(m=5) & Beta & Cort & Bagged Cort\\
\midrule
\addlinespace[0.3em]
\multicolumn{7}{l}{\textbf{Kendall Tau}}\\
\hspace{1em}$\tau_{1,2}$ & 0.006 & 0.005 & 0.004 & 0.014 & 0 & -0.010\\
\addlinespace[0.3em]
\multicolumn{7}{l}{\textbf{Spearman Rho}}\\
\hspace{1em}$\rho_{1,2}$ & 0.010 & 0.011 & 0.009 & 0.021 & 0 & -0.014\\
\bottomrule
\end{tabu}
\end{table}


==> recoveryourself_table_bagging_result.tex <==
\begin{table}[H]

\caption{\label{tab:recoveryourself_table_bagging_result}Results of the bagging of each model on Dataset \ref{data:recoveryourself}}
\centering
\begin{tabu} to \linewidth {>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X}
\toprule
  & Empirical & Cb(m=10) & Cb(m=5) & Beta & Cort\\
\midrule
$\hat{J}(\hat{c}_{\Gras{\omega}})$ & 0.002 & -3.16 & -2.37 & -2.98 & \textbf{-4.81}\\
$\hat{K}(\hat{c}_{\Gras{\omega}})$ & Inf & -1.06 & -0.743 & \textbf{-1.18} & -0.837\\
$\hat{M}(\hat{c}_{\Gras{\omega}})$ & \textbf{8.72e-06} & 4.13e-05 & 0.000281 & 1.58e-05 & 0.000633\\
$\hat{N}(\hat{c}_{\Gras{\omega}})$ & \textbf{-0.0277} & -0.0277 & -0.0275 & -0.0277 & -0.0262\\
\bottomrule
\end{tabu}
\end{table}


==> recoveryourself_table_cramer.tex <==
\begin{table}[H]

\caption{\label{tab:recoveryourself_table_cramer}$\hat{P}$ error statistics for Dataset \ref{data:recoveryourself}}
\centering
\begin{tabu} to \linewidth {>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X}
\toprule
  & Empirical & Cb(m=10) & Cb(m=5) & Beta & Cort & Cort Forest\\
\midrule
Mean & 8.59e-05 & 8.63e-05 & 3.11e-04 & \textbf{7.72e-05} & 7.85e-05 & 1.80e-03\\
Sd & 6.58e-05 & 4.74e-05 & 6.72e-05 & 6.21e-05 & \textbf{3.57e-05} & 3.10e-03\\
\bottomrule
\end{tabu}
\end{table}


==> recoveryourself_table_dep_mes.tex <==
\begin{table}[H]

\caption{\label{tab:recoveryourself_table_dep_mes}Obtained dependence measures of several models on Dataset \ref{data:recoveryourself}}
\centering
\begin{tabu} to \linewidth {>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X>{\raggedright}X}
\toprule
  & Empirical & Cb(m=10) & Cb(m=5) & Beta & Cort & Bagged Cort\\
\midrule
\addlinespace[0.3em]
\multicolumn{7}{l}{\textbf{Kendall Tau}}\\
\hspace{1em}$\tau_{1,2}$ & -0.534 & -0.515 & -0.465 & -0.527 & -0.525 & -0.393\\
\addlinespace[0.3em]
\multicolumn{7}{l}{\textbf{Spearman Rho}}\\
\hspace{1em}$\rho_{1,2}$ & -0.773 & -0.757 & -0.697 & -0.766 & -0.762 & -0.604\\
\bottomrule
\end{tabu}
\end{table}

